A Faster Fourier Transform? Computing Small-Scale Power Spectra and Bispectra for Cosmological Simulations in $\mathcal{O}(N^2)$ Time

We present $\mathcal{O}(N^2)$ estimators for the small-scale power spectrum and bispectrum in cosmological simulations. In combination with traditional methods, these allow spectra to be efficiently computed across a vast range of scales, requiring orders of magnitude less computation time than Fast Fourier Transform based approaches alone. These methods are applicable to any tracer; simulation particles, halos or galaxies, and take advantage of the simple geometry of the box and periodicity to remove almost all dependence on large random particle catalogs. By working in configuration-space, both power spectra and bispectra can be computed via a weighted sum of particle pairs up to some radius, which can be reduced at larger $k$, leading to algorithms with decreasing complexity on small scales. These do not suffer from aliasing or shot-noise, allowing spectra to be computed to arbitrarily large wavenumbers. The estimators are rigorously derived and tested against simulations, and their covariances discussed. The accompanying code, HIPSTER, has been publicly released, incorporating these algorithms. Such estimators will be of great use in the analysis of large sets of high-resolution simulations.

==> old_paper.tex <==
%\oliver{Think about how 2PCF and power spectrum covariances simplify in the periodic limit. Each integral will have a decoupling V at least, reducing the dimensionality.}

\section{Estimators for $P(\vec k)$}
We here derive the configuration-space estimators for the power in N-body simulations, analogous to the forms presented in \citet{real-space-power} for arbitrary survey geometries. For a cubic simulation with periodic boundaries, the 2PCF estimator is given by
\beq
    \xi(\vec r) = \frac{DD(\vec r)}{RR(\vec r)}-1
\eeq
which is equivalent to the \citet{1993ApJ...412...64L} estimator if the boundaries are periodic (since $DR(\vec r) = RR(\vec r)$). For a box with mean number density $n$, the counts are given (in continuous form) by integrals over the survey volume $V$;
\beq
    DD(\vec r) &=& \int_V d^3\vec r_i\,d^3\vec r_j\,n_g(\vec r_i)n_g(\vec r_j)\delta^{(D)}(\vec r - (\vec r_i - \vec r_j))\\\nonumber
    RR(\vec r) &=& n^2\int_V d^3\vec r_i\,d^3\vec r_j\,\delta^{(D)}(\vec r - (\vec r_i- \vec r_j) = n^2V\int_V d^3\vec x\,\delta^{(D)}(\vec r-\vec x) = n^2V
\eeq
for Dirac delta function $\delta^{(D)}$ and galaxy density function $n_g$ (simply a sum over delta functions at each of $N$ galaxy positions), where we assume periodicity in the final line and substitute $\vec x = \vec r_i- \vec r_j$. We here assume that $\vec r$ lies inside the survey geometry (i.e. that $|r_i| < L/2$ for $i\in\{1,2,3\}$ and box-size $L$). The power spectrum is simply the Fourier transform of the 2PCF;
\beq
    P(\vec k) &=& \frac{1}{n^2V}\int_V d^3\vec r\,e^{i\vec k\cdot\vec r}\int_V d^3\vec r_i\,d^3\vec r_j\,n_g(\vec r_i)n_g(\vec r_j)\delta^{(D)}(\vec r - (\vec r_i - \vec r_j)) - \int_V d^3\vec r\,e^{i\vec k\cdot\vec r}\\\nonumber
    &=& \frac{1}{n^2V}\int d^3\vec r_i\,d^3\vec r_j\,e^{i\vec k\cdot(\vec r_i-\vec r_j)}n_g(\vec r_i)n_g(\vec r_j) - \int_V d^3\vec r\,e^{i\vec k\cdot\vec r}
\eeq
integrating over the Delta function and again invoking periodicity. Using the galaxy density definition
\beq
    n_g(\vec r) = \sum_{i\in D} \delta^{(D)}(\vec r - \vec r_i)
\eeq
(where $i$ runs through all $N$ galaxies in the dataset) we obtain
\beq
    P(\vec k) = \frac{1}{n^2V}\sum_{i\in D}\sum_{j\in D,\,j\neq i}e^{i\vec k\cdot(\vec r_i-\vec r_j)} - \int_V d^3\vec r\,e^{i\vec k\cdot\vec r},
\eeq
excluding self-counts to avoid shot-noise contributions to the final power. As in \citet{real-space-power}, one can introduce a (spherical) pair-separation window function $W(|\vec r|; R_0)$, which has support for $|\vec r|\in[0,R_0]$ using truncation radius $R_0$. We here utilize the form suggested in \citet{real-space-power};
\beq\label{eq: window_defn}
    W(\vec r; R_0) &\equiv& f\left(\frac{|\vec r|}{R_0}\right)\\\nonumber
    f(x) &=& \begin{cases} 1 & \text{if } 0\leq x < 1/2 \\ 1-8\left(2x - 1 \right)^3 + 8 \left(2x - 1\right)^4& \text{if }1/2\leq x<3/4\\ -64\left(x-1\right)^3 - 128\left(x-1\right)^4 & \text{if } 3/4\leq x< 1\\ 0 & \text {else}\end{cases}
\eeq
which is smooth up to the third derivative at break-points, with $W=1$ for $r<R_0/2$. This modifies the power spectrum to the form
\beq
    P(\vec k; R_0) = \frac{1}{n^2V}\sum_{i\in D}\sum_{j\in D,\,j\neq i}e^{i\vec k\cdot(\vec r_i-\vec r_j)}W(|\vec r_i-\vec r_j|; R_0) - \int_Vd^3\vec r\,e^{i\vec k\cdot\vec r}W(|\vec r|; R_0).
\eeq
Note that the final term is simply the Fourier transform of $\Omega(\vec r)W(|\vec r|;R_0)$ where $\Omega(\vec r)$ is unity if $\vec r$ is in the box and zero else. The pair-separation window $W$ convolves the true box-power $P(\vec k)$ with the Fourier-space window $\widetilde{W}(|\vec k|;R_0)$; which has characteristic width in  $k$-space of $\approx 5/R_0$ and a strong fall-off at higher $k$. The inclusion of $W$ allows us to consider only pairs with separations up to $R_0$; this greatly expedites computation of small-scale power. Including effects from both the cubic box selection function and $W$, the true power spectrum is convolved with the function $\mathcal{F}\left[\Omega(\vec r) W(\vec r;R_0)\right](\vec k) = \left[\widetilde{\Omega}\ast\widetilde{W}_{R_0}\right](\vec k)$

\section{Multipoles of $P(\vec k)$}
Now consider the power spectrum multipoles defined for a cubic box as
\beq
    P_\ell(k;R_0) \equiv (2\ell+1)\int \frac{d\Omega_k}{4\pi} P(\vec k;R_0)L_\ell(\hat{\vec k}\cdot\hat{\vec z})
\eeq
where $\hat{\vec z}$ is the line-of-sight (LoS) direction and $L_\ell$ is the Legendre polynomial of order $\ell$. We note that
\beq
    \int \frac{d\Omega_k}{4\pi} e^{i\vec k\cdot\vec r}L_\ell(\hat{\vec k}\cdot\hat{\vec z}) &=& \sum_{\ell'=0}^\infty i^{\ell'}(2\ell'+1)j_{\ell'}(kr)\int \frac{d\Omega_k}{4\pi}L_\ell(\hat{\vec k}\cdot\hat{\vec z})L_{\ell'}(\hat{\vec k}\cdot\hat{\vec r})\\\nonumber
    &=& \sum_{\ell'=0}^\infty i^{\ell'}(2\ell'+1)j_{\ell'}(kr)\int\frac{d\Omega_k}{4\pi}\sum_{m=-\ell}^\ell\sum_{m'=-\ell'}^{\ell'}\frac{(4\pi)^2}{(2\ell'+1)(2\ell+1)}Y^{}_{\ell m}(\hat{\vec k})Y^{*}_{\ell m}(\hat{\vec z})Y^{*}_{\ell'm'}(\hat{\vec k})Y^{}_{\ell'm'}(\hat{\vec r})\\\nonumber
    &=& i^\ell j_\ell(kr)L_\ell(\hat{\vec r}\cdot\hat{\vec z}),
\eeq
where $j_\ell$ and $Y_{\ell m}$ are the $\ell$-th order spherical Bessel functions of the first kind and spherical harmonics respectively. This is derived via the plane wave expansion \citep[Eq.\,16.63]{arfken2013mathematical}, spherical harmonic addition theorem \citep[Eq.\,14.30.9]{nist_dlmf} and spherical harmonic orthonormality \citep[Eq.\,14.30.8]{nist_dlmf}. The power multipoles may hence be written
\beq\label{eq: power-pair-count-full}
    P_\ell(k;R_0) = \frac{i^\ell(2\ell+1)}{n^2V}\sum_{i\in D}\sum_{j\in D,\,j\neq i} j_\ell(k|\vec r_i-\vec r_j|)W(|\vec r_i-\vec r_j|; R_0)L_\ell(\widehat{(\vec r_i-\vec r_j)}\cdot\hat{\vec z}) - i^\ell(2\ell+1)\int_Vd^3\vec r\,j_\ell(k|\vec r|)W(|\vec r|;R_0)L_\ell(\hat{\vec r}\cdot\hat{\vec z}).
\eeq
Note that this is simply a pair count of galaxies $i$ and $j$ in the simulation, weighted by a kernel dependent on $\ell$. For convenience, we define the kernel
\beq
    A_\ell(r,\mu;k,R_0) \equiv i^\ell (2\ell+1) j_\ell(kr)W(r;R_0)L_\ell(\mu)
\eeq
where $r = |\vec r$ and $\mu$ is the cosine of the angle between $\vec r$ and the LoS $\hat{\vec z}$. This gives the estimator in the form of a sum over pairs (without self-counts)
\beq
    \widehat{P}_\ell(k;R_0) = \frac{1}{n^2V}\sum_{i\in D}\sum_{j\in D,\,j\neq i}A_\ell(r_{ij},\mu_{ij};k,R_0) - P_\ell^\mathrm{geom}(k;R_0)
\eeq
where $r_{ij} = |\vec r_i-\vec r_j|$ and $\mu_{ij} = \widehat{(\vec r_i-\vec r_j)}\cdot\hat{\vec{z}}$, defining $P_\ell^\mathrm{geom}$ as the second term in Eq.\,\ref{eq: power-pair-count-full}, which is a correction for the cubic box geometry. In the limit of $R_0\leq L/2$ (where the domain of $W(\vec r;R_0)$ does not intersect the survey boundary), this may be simplified to
\beq
    P_\ell^\mathrm{geom}(k;R_0) = 4\pi i^\ell(2\ell+1)\int_0^{R_0} r^2dr\,j_\ell(kr)W(r;R_0)\int_0^1d\mu\,L_\ell(\mu) = 4\pi\delta^{(K)}_{\ell 0}\int_0^{R_0}r^2dr\,j_0(kr)W(r;R_0) 
\eeq
for Kronecker delta $\delta^{(K)}$, noting that this only corrects the monopole power. This is simply identified as the Fourier transform of the pair-separation window function $W(r;R_0)$. In the limit where $R_0\geq L\sqrt{3}$, $W=1$ everywhere inside the box, and $P_\ell^\mathrm{geom}$ is simply the $\ell$-th multipole of the Fourier transform of a cubic top-hat function.

\section{Binning in $k$-space}
The above pair-count estimator may be extended to allow for binning in $k$-space, where the estimate in bin $a$ is defined as
\beq
    P^a_\ell(R_0) = \frac{1}{\Delta_k^a}\int_{k_{a,\mathrm{min}}}^{k_{a,\mathrm{max}}} k^2dk\,P_\ell(k;R_0)
\eeq
where $\Delta_k^a = k_{a,\mathrm{max}}^3-k_{a,\mathrm{min}}^3$. This gives the full pair-count configuration-space estimator
\beq
    \widehat{P}_\ell^a(R_0) = \frac{1}{n^2V}\sum_{i\in D}\sum_{j\in D,\,j\neq i}A^a_\ell(r_{ij},\mu_{ij};R_0) - P_{\ell,a}^\mathrm{geom}(R_0)
\eeq
defining
\beq
    A_\ell^a(r,\mu;R_0) &=& i^\ell(2\ell+1)W(r;R_0)L_\ell(\mu)Q^a(r)\\\nonumber
    P_{\ell,a}^\mathrm{geom}(R_0) &=& i^\ell(2\ell+1)\int_Vd^3\vec r\,W(|\vec r|;R_0)L_\ell(\hat{\vec r}\cdot\hat{\vec z})Q^a(|\vec r|)
\eeq
for bin-averaged Bessel function
\beq
    Q^a(r) = \frac{1}{\Delta_k^a}\int_{k_{a,\mathrm{min}}}^{k_{a,\mathrm{max}}} k^2dk\,j_\ell(kr).
\eeq
This estimator has complexity $\mathcal{O}(Nn\times R_0^3\times N_k)$ for $N$ particles with number density $n$ in $N_k$ $k$-space bins (assuming $R_0\leq L/2$), since we count all $N$ primary particles and $n\times 4\pi R_0^3/3$ secondary particles. Since the window function $W(r;R_0)$ smooths $P(\vec k)$ with characteristic scale $\Delta k\sim 5/R_0$, if linear binning is required, the bin-width should not be significantly below $5/R_0$ to avoid large mode mixing between bins. For logarithmic binning of fixed $\Delta\log k$, it is desirable to set $R_0 \propto 1/k$, implying that at large galaxy-pair separation, we only consider contributions to the small $k$ bins.

